Multi-Purposing Domain Adaptation Discriminators for Pseudo Labeling Confidence

Often domain adaptation is performed using a discriminator (domain classifier) to learn domain-invariant feature representations so that a classifier trained on labeled source data will generalize well to unlabeled target data. A line of research stemming from semi-supervised learning uses pseudo labeling to directly generate "pseudo labels" for the unlabeled target data and trains a classifier on the now-labeled target data, where the samples are selected or weighted based on some measure of confidence. In this paper, we propose multi-purposing the discriminator to not only aid in producing domain-invariant representations but also to provide pseudo labeling confidence.

==> acmart-preload-hook.tex <==
% - load scrextend before hyperrref for footref in table https://tex.stackexchange.com/a/95905
% - Allow wrapping long URLs https://tex.stackexchange.com/a/3034
\let\LoadClassOrig\LoadClass
\renewcommand\LoadClass[2][]{\LoadClassOrig[#1]{#2}%
\PassOptionsToPackage{hyphens}{url}
\usepackage{scrextend}}

